Toward Strategy Identification and Subtask Decomposition In Task Exploration

This research builds on work in anticipatory human-machine interaction, a subfield of human-machine interaction where machines can facilitate advantageous interactions by anticipating a user's future state. The aim of this research is to further a machine's understanding of user knowledge, skill, and behavior in pursuit of implicit coordination. A task explorer pipeline was developed that uses clustering techniques, paired with factor analysis and string edit distance, to automatically identify key global and local strategies that are used to complete tasks. Global strategies identify generalized sets of actions used to complete tasks, while local strategies identify sequences that used those sets of actions in a similar composition. Additionally, meaningful subtasks of various lengths are identified within the tasks. The task explorer pipeline was able to automatically identify key strategies used to complete tasks and encode user runs with hierarchical subtask structures. In addition, a Task Explorer application was developed to easily review pipeline results. The task explorer pipeline can be easily modified to any action-based time-series data and the identified strategies and subtasks help to inform humans and machines on user knowledge, skill, and behavior.

==> abs.tex <==
This research builds on work in anticipatory human-machine interaction, a subfield of human-machine interaction where machines can facilitate advantageous interactions by anticipating a user's future state. The aim of this research is to further a machine's understanding of user knowledge, skill, and behavior in pursuit of implicit coordination. A task explorer pipeline was developed that uses clustering techniques, paired with factor analysis and string edit distance, to automatically identify key global and local strategies that are used to complete tasks. Global strategies identify generalized sets of actions used to complete tasks, while local strategies identify sequences that used those sets of actions in a similar composition. Additionally, meaningful subtasks of various lengths are identified within the tasks. The task explorer pipeline was able to automatically identify key strategies used to complete tasks and encode user runs with hierarchical subtask structures. In addition, a Task Explorer application was developed to easily review pipeline results. The task explorer pipeline can be easily modified to any action-based time-series data and the identified strategies and subtasks help to inform humans and machines on user knowledge, skill, and behavior.

{\bf Keywords:} Anticipatory HMI, HMI, Task Exploration, Strategy Identification, Subtask Identification, Clustering, String Edit Distance, Factor Analysis



==> ack.tex <==


I am deeply indebted to Dr. Tom Austin for his guidance and invaluable feedback. This endeavor would also not have been possible without Dr. Grit Denker, who inspired this research and has continuously offered her incredible knowledge and expertise. Additionally, I would like to express my deepest appreciation to Dr. Jon Pearce for his imperative insights and unwavering support in my professional ambitions. 

I am also grateful to Dr. Huascar Sanchez for his essential subject-matter expertise and for inspiring me to think innovatively.

Lastly, I am also thankful for my parents and my fiancée, who provided both distractions when needed and constant encouragement throughout this journey.



==> appB.tex <==






==> keep_examples.tex <==
Was 15 pages without me writing anything

\chapter{Literature Review\label{chap:blah}}

Some more important stuff

\section{Figures}

Figure~\ref{fig:encrypted_virus} has been typeset so that it
occupies half the width of text on a page ({\tt width=0.5}). Note the 
symbolic cross-reference, that is, you simple \verb+\ref{fig:encrypted_virus}+
to obtain the appropriate number for Figure~\ref{fig:encrypted_virus}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.5\textwidth]{images/encrypted_virus.jpg}
\caption{Encrypted virus before and after decryption.} 
\label{fig:encrypted_virus}
\end{figure}

If you move things around, insert or delete text, Figure~\ref{fig:encrypted_virus}
will still give you the correct number. This is a very handy feature.


\section{Tables}

Table~\ref{tab:19} 
shows some interesting stuff. I hope you enjoy it.

\begin{table}[htb]
\caption{MysteryTwister Zodiac Challenge\label{tab:19}}
\begin{center}
\begin{tabular}{c|lc}\hline\hline
Case & \multicolumn{1}{c}{Description} & Percentage\\ \hline
1F & Fast outer hill climb and English stats & 13.00\% \\
1S & Slow outer hill climb and English stats & \phantom{0}4.00\% \\
2F & Fast outer hill climb and Zodiac~408 stats & 70.00\% \\
2S & Slow outer hill climb and Zodiac~408 stats & 84.00\% \\ \hline\hline
\end{tabular}
\end{center}
\end{table}


\section{Citations}

References are cited using the \verb+\cite+ command. For example,
see~\cite{harden} for information on the Zodiac killer. You can include more than one 
reference in a single citation, like this~\cite{harden,bib1,basa,bib3,bib2,glurk,bib7,bib10,bib11}
or this~\cite{bibAC,bib17}.


\section{The Last Word}

There are a lot of other uses for symbolic cross-referencing. For example, this chapter
title has a label so I can refer to Chapter~\ref{chap:blah} (as I just did).
My recommendation is that you include a label with anything and everything that 
is numbered. If it has a number, there is a good chance that you will
refer to it at some point.

Finally, note that you need to \LaTeX\ a file at least twice (three times to
be safe) without changing anything to be sure that the numbering is correct.
Why is that? Good question.
When you \LaTeX\ your document, various auxiliary files are created. Most of these files contain
information related to cross-references that appear in your {\tt .tex} file (or files). The next time you 
\LaTeX\ your document, the information from the previous run is read from
these auxiliary files. Consequently, after making changes to any {\tt .tex}
file, you will need to \LaTeX\ your document at least twice to be sure that the
cross-reference information is updated in the resulting pdf. In fact, you should
run \LaTeX\ three consecutive times to be certain that cross-references are correct.



\chapter{Methods}

For this thesis
format, you \LaTeX\ the file {\tt thesis.tex}. 
But first, you
need to make some modifications to {\tt thesis.tex}.
The title of your report, committee members, etc.,
are specified in {\tt thesis.tex}. All of the things that
you need to modify are indicated by comments beginning with five consecutive asterisks, 
so search for ``*****'' in {\tt thesis.tex} and make the necessary changes.

You put the actual content of your report 
in the following files:
\begin{itemize}
\item {\tt abs.tex} --- abstract
\item {\tt ack.tex} --- acknowledgements
\item {\tt chap1.tex}, {\tt chap2.tex}, and so on --- chapters
\item {\tt bib.tex} --- references
\item {\tt appA.tex}, {\tt appB.tex}, and so on --- appendices (if any)
\end{itemize}


\chapter{Results}

I do not usually talk about myself, but when I do, I talk about my cat.\\

In April 2010, the American economy was gripped by its most severe economic crisis in at least a generation.  There was in a deep recession.  It was in this climate that a great savior was born; her name is Muffins.  

\begin{figure}[ht!]
\centering
\includegraphics[width=90mm]{./images/muffins.jpg}
\caption{A Week Old Muffins}
\end{figure}

She is the first cat I have ever owned.  She is a purebred Siberian.  Her interests include: \\
\begin{itemize}
	\item Sleeping
	\item Grooming herself
	\item Twister
\end{itemize}

The reason I chose to get a Siberian cat is because they are purported (perhaps dubiously) to be hypoallergenic. They are also a very healthy breed as they were more recently domesticated.\

\section{Career Goals}

I am impressed by the ground working done by the renowned dog rehabilitator Cesar Millan, host of the critically acclaimed television show "Dog Whisperer." It is my hope that I could have an equally successful television program which I will entail "Cat Telepathist"  where I will rehabilitate troubled and stray cats through the power of extrasensory perception (ESP).

If my "Cat Telepathist" show were not to find a niche with audiences, my second television show is modeled after the former television show "Crossing Over with John Edward." \cite{calderwood} I plan to call the show "You have Cat to be Kitten Me with Zayd Hammoudeh" and will be used to give grieving families the opportunity to communicate with their deceased feline family members.

Other TV show ideas I would like to pursue include:
\begin{itemize}
	\item Cat Mustache Aficionado - A daily discussion of cat whiskers.
	\item Alien vs. Predator vs. Cat - It is like the movie "Alien vs. Predator" but instead of it being a two party battle, it is a triple threat match with a cat.
	\item Cat Hoarders - A show where we do an intervention with a cat that hoards some type of item.
\end{itemize}


\chapter{Results}

I do not usually talk about myself, but when I do, I talk about my cat.\\

In April 2010, the American economy was gripped by its most severe economic crisis in at least a generation.  There was in a deep recession.  It was in this climate that a great savior was born; her name is Muffins.  

\begin{figure}[ht!]
\centering
\includegraphics[width=90mm]{./images/muffins.jpg}
\caption{A Week Old Muffins}
\end{figure}

She is the first cat I have ever owned.  She is a purebred Siberian.  Her interests include: \\
\begin{itemize}
	\item Sleeping
	\item Grooming herself
	\item Twister
\end{itemize}

The reason I chose to get a Siberian cat is because they are purported (perhaps dubiously) to be hypoallergenic. They are also a very healthy breed as they were more recently domesticated.\

\section{Career Goals}

I am impressed by the ground working done by the renowned dog rehabilitator Cesar Millan, host of the critically acclaimed television show "Dog Whisperer." It is my hope that I could have an equally successful television program which I will entail "Cat Telepathist"  where I will rehabilitate troubled and stray cats through the power of extrasensory perception (ESP).

If my "Cat Telepathist" show were not to find a niche with audiences, my second television show is modeled after the former television show "Crossing Over with John Edward." \cite{calderwood} I plan to call the show "You have Cat to be Kitten Me with Zayd Hammoudeh" and will be used to give grieving families the opportunity to communicate with their deceased feline family members.

Other TV show ideas I would like to pursue include:
\begin{itemize}
	\item Cat Mustache Aficionado - A daily discussion of cat whiskers.
	\item Alien vs. Predator vs. Cat - It is like the movie "Alien vs. Predator" but instead of it being a two party battle, it is a triple threat match with a cat.
	\item Cat Hoarders - A show where we do an intervention with a cat that hoards some type of item.
\end{itemize}

\begin{itemize}
\item[Space Ghost:]
Everybody wants to be Space Ghost\\ 
Everybody near and far\\
Hey, ma, look at me, I'm on TV\\
Everybody wants to be a star\\
I'm Space Ghost, Mr. Space Ghost\\
I've got big muscles, And I can dance\\
When Zorak tries to bug me, I zap him with my power bands
\item[Zorak:]
Uhhhh$\ldots$ I don't think that will be necessary
\item[Space Ghost:]
I think I'll zap him with my power bands\\
On Saturn and Jupiter and Neptune, too\\
I've been hearing it from coast to coast\\
I'd give anything, If for just one day\\
I could be a super hero like Space Ghost
\item[Zorak:]
Ugghh$\ldots$ Why would anyone want to be Space Ghost?
\item[Space Ghost:]
Everybody wants to be just like me!
\end{itemize}
